Root Cause Explanation of Outliers under Noisy Mechanisms

Identifying root causes of anomalies in causal processes is vital across disciplines. Once identified, one can isolate the root causes and implement necessary measures to restore the normal operation. Causal processes are often modelled as graphs with entities being nodes and their paths/interconnections as edge. Existing work only consider the contribution of nodes in the generative process, thus can not attribute the outlier score to the edges of the mechanism if the anomaly occurs in the connections. In this paper, we consider both individual edge and node of each mechanism when identifying the root causes. We introduce a noisy functional causal model to account for this purpose. Then, we employ Bayesian learning and inference methods to infer the noises of the nodes and edges. We then represent the functional form of a target outlier leaf as a function of the node and edge noises. Finally, we propose an efficient gradient-based attribution method to compute the anomaly attribution scores which scales linearly with the number of nodes and edges. Experiments on simulated datasets and two real-world scenario datasets show better anomaly attribution performance of the proposed method compared to the baselines. Our method scales to larger graphs with more nodes and edges.

==> discuss.tex <==
Our aim is to variationally hyper-encode networks, in which all network
weights $\theta$ is encoded into $u$. Thus it is considered a lossless
compression strategy where the HyperVAE compress a whole family of
networks that parametrize the parameters of distributions across datasets.
The model code length and data misfits are minimized using HyperVAE,
therefore the whole code length is minimized.

This is in contrast to the lossy compression strategy \cite{chen2016variational}
where local information of images are freely decoded independent of
the compressed information. We leave this direction for future research
which include descendants of hypernetworks \cite{ha2016hypernetworks}
which utilize independent local networks.

